Propagation from Deceptive News Sources: Who Shares, How Much, How Evenly, and How Quickly?

As people rely on social media as their primary sources of news, the spread of misinformation has become a significant concern. In this large-scale study of news in social media we analyze eleven million posts and investigate propagation behavior of users that directly interact with news accounts identified as spreading trusted versus malicious content. Unlike previous work, which looks at specific rumors, topics, or events, we consider all content propagated by various news sources. Moreover, we analyze and contrast population versus sub-population behaviour (by demographics) when spreading misinformation, and distinguish between two types of propagation, i.e., direct retweets and mentions. Our evaluation examines how evenly, how many, how quickly, and which users propagate content from various types of news sources on Twitter. Our analysis has identified several key differences in propagation behavior from trusted versus suspicious news sources. These include high inequity in the diffusion rate based on the source of disinformation, with a small group of highly active users responsible for the majority of disinformation spread overall and within each demographic. Analysis by demographics showed that users with lower annual income and education share more from disinformation sources compared to their counterparts. News content is shared significantly more quickly from trusted, conspiracy, and disinformation sources compared to clickbait and propaganda. Older users propagate news from trusted sources more quickly than younger users, but they share from suspicious sources after longer delays. Finally, users who interact with clickbait and conspiracy sources are likely to share from propaganda accounts, but not the other way around.

==> figs/lorenz_gini_example.tex <==
\usepgfplotslibrary{fillbetween}
\begin{tikzpicture}
\begin{axis}[
%enlargelimits=0.01,
%hide axis,
%axis lines*=left,
axis lines = left,
clip=false,
height=2.25in, width=2.25in,
xlabel style={yshift=0.05in,align=center}, 
ylabel style={yshift=-0.1in,align=center},
legend cell align={left},
legend style={at={(.5,-.25)},%at={(2,1)},
	anchor=north,legend columns=-1,draw=none,fill=none,font=\small},%column sep=.05cm,
%legend style={at={(1.6,1)},%at={(2,1)},
%anchor=north,legend columns=1,column sep=.1cm,draw=none,font=\small},
xlabel={cumulative \% active users \\ \textcolor{gray!50!black}{(cumulative \% population)}},
ylabel={\% propagation (tweets shared)\\ \textcolor{gray!50!black}{(\% income)}},
xmin=0-.1,xmax=1.1,ymin=0-.1,ymax=1.1,
xtick = {0,.25,.5,.75,1},xticklabels ={0,25,50,75,100},%xticklabels ={{0~~~~~~},25,50,75,100},
ytick = {0,.25,.5,.75,1},yticklabels ={0,25,50,75,100},%yticklabels ={,25,50,75,100},
xtick align=center, 
ytick align=center, 
title ={Propagation Inequality\\ \textcolor{gray!50!black}{(Income Inequality)}}, title style = {yshift= -.1in, xshift=-.1in,align=center},
%nodes near coords,
%nodes near coords align={vertical},
%title = Retweet-diffusion as a function of the proportion of users retweeting %Retweet-User Inequality Curves
]


%\draw[black!50] (175,20) node[anchor=south,color=black] {\normalsize $G = {\dfrac{a_1}{a_1+a_2}} $} ;

%Perfect Equality
\addplot[black,no marks,thick, name path=perfectEquality] coordinates {
	(0,0) (1,1)
};  
%\draw[black] (axis cs:(0.5,0.5) node[anchor=south,rotate=45] {  {\tiny Lorenz Curve of Perfect Equality} };
 
%Perfect Inequality
\addplot[black,no marks,very thick,densely dotted] coordinates {
	(0.001,0.001) 
	(1,0.001) (1,1)
};

%\draw[black, thick] (.5,.5) -- (.4,.7) node[anchor=south,color=black] {{\small Perfect Equality}} ;

\draw[black!50] (75,55) node[color=black] {\normalsize $a_1$} ;
\draw[black!50] (95,20) node[anchor=south,color=black] {\normalsize$a_2$} ;

% propaganda with mentions
\addplot[no marks,black, dashed, thick, name path=lorenz] coordinates {
	(1,1)
	% (2016+) propaganda, Gini:0.527386049892, Palma:3.13816751094
	( 1 - 0.00999947940235 , 1 - 0.251670554094 )  ( 1 - 0.0199989588047 , 1 - 0.311754693227 )  ( 1 - 0.0299984382071 , 1 - 0.353967063288 )  ( 1 - 0.0399979176094 , 1 - 0.387767161445 )  ( 1 - 0.0499973970118 , 1 - 0.415830500518 )  ( 1 - 0.0599968764141 , 1 - 0.4404222386 )  ( 1 - 0.0699963558165 , 1 - 0.461292880017 )  ( 1 - 0.0799998398161 , 1 - 0.481728545424 )  ( 1 - 0.0899993192185 , 1 - 0.498123037478 )  ( 1 - 0.0999987986208 , 1 - 0.514517529533 )  ( 1 - 0.109998278023 , 1 - 0.530912021588 )  ( 1 - 0.119997757426 , 1 - 0.543518118802 )  ( 1 - 0.129997236828 , 1 - 0.555813987843 )  ( 1 - 0.13999671623 , 1 - 0.568109856885 )  ( 1 - 0.149996195633 , 1 - 0.580405725926 )  ( 1 - 0.159999679632 , 1 - 0.592706519223 )  ( 1 - 0.169999159035 , 1 - 0.604337613607 )  ( 1 - 0.179998638437 , 1 - 0.612534859634 )  ( 1 - 0.189998117839 , 1 - 0.620732105662 )  ( 1 - 0.199997597242 , 1 - 0.628929351689 )  ( 1 - 0.209997076644 , 1 - 0.637126597717 )  ( 1 - 0.219996556046 , 1 - 0.645323843744 )  ( 1 - 0.229996035449 , 1 - 0.653521089771 )  ( 1 - 0.239999519448 , 1 - 0.661721618637 )  ( 1 - 0.249998998851 , 1 - 0.669918864664 )  ( 1 - 0.259998478253 , 1 - 0.678116110692 )  ( 1 - 0.269997957655 , 1 - 0.686313356719 )  ( 1 - 0.279997437058 , 1 - 0.694510602747 )  ( 1 - 0.28999691646 , 1 - 0.702707848774 )  ( 1 - 0.299996395862 , 1 - 0.710905094802 )  ( 1 - 0.309999879862 , 1 - 0.717180239287 )  ( 1 - 0.319999359264 , 1 - 0.721278862301 )  ( 1 - 0.329998838667 , 1 - 0.725377485315 )  ( 1 - 0.339998318069 , 1 - 0.729476108328 )  ( 1 - 0.349997797471 , 1 - 0.733574731342 )  ( 1 - 0.359997276874 , 1 - 0.737673354355 )  ( 1 - 0.369996756276 , 1 - 0.741771977369 )  ( 1 - 0.379996235679 , 1 - 0.745870600383 )  ( 1 - 0.389999719678 , 1 - 0.749970864815 )  ( 1 - 0.399999199081 , 1 - 0.754069487829 )  ( 1 - 0.409998678483 , 1 - 0.758168110842 )  ( 1 - 0.419998157885 , 1 - 0.762266733856 )  ( 1 - 0.429997637288 , 1 - 0.766365356869 )  ( 1 - 0.43999711669 , 1 - 0.770463979883 )  ( 1 - 0.449996596092 , 1 - 0.774562602897 )  ( 1 - 0.459996075495 , 1 - 0.77866122591 )  ( 1 - 0.469999559494 , 1 - 0.782761490343 )  ( 1 - 0.479999038897 , 1 - 0.786860113356 )  ( 1 - 0.489998518299 , 1 - 0.79095873637 )  ( 1 - 0.499997997701 , 1 - 0.795057359384 )  ( 1 - 0.509997477104 , 1 - 0.799155982397 )  ( 1 - 0.519996956506 , 1 - 0.803254605411 )  ( 1 - 0.529996435908 , 1 - 0.807353228424 )  ( 1 - 0.539999919908 , 1 - 0.811453492857 )  ( 1 - 0.54999939931 , 1 - 0.81555211587 )  ( 1 - 0.559998878713 , 1 - 0.819650738884 )  ( 1 - 0.569998358115 , 1 - 0.823749361898 )  ( 1 - 0.579997837517 , 1 - 0.827847984911 )  ( 1 - 0.58999731692 , 1 - 0.831946607925 )  ( 1 - 0.599996796322 , 1 - 0.836045230938 )  ( 1 - 0.609996275725 , 1 - 0.840143853952 )  ( 1 - 0.619999759724 , 1 - 0.844244118384 )  ( 1 - 0.629999239127 , 1 - 0.848342741398 )  ( 1 - 0.639998718529 , 1 - 0.852441364412 )  ( 1 - 0.649998197931 , 1 - 0.856539987425 )  ( 1 - 0.659997677334 , 1 - 0.860638610439 )  ( 1 - 0.669997156736 , 1 - 0.864737233452 )  ( 1 - 0.679996636138 , 1 - 0.868835856466 )  ( 1 - 0.689996115541 , 1 - 0.87293447948 )  ( 1 - 0.69999959954 , 1 - 0.877034743912 )  ( 1 - 0.709999078943 , 1 - 0.881133366926 )  ( 1 - 0.719998558345 , 1 - 0.885231989939 )  ( 1 - 0.729998037747 , 1 - 0.889330612953 )  ( 1 - 0.73999751715 , 1 - 0.893429235966 )  ( 1 - 0.749996996552 , 1 - 0.89752785898 )  ( 1 - 0.759996475954 , 1 - 0.901626481994 )  ( 1 - 0.769999959954 , 1 - 0.905726746426 )  ( 1 - 0.779999439356 , 1 - 0.90982536944 )  ( 1 - 0.789998918759 , 1 - 0.913923992453 )  ( 1 - 0.799998398161 , 1 - 0.918022615467 )  ( 1 - 0.809997877563 , 1 - 0.922121238481 )  ( 1 - 0.819997356966 , 1 - 0.926219861494 )  ( 1 - 0.829996836368 , 1 - 0.930318484508 )  ( 1 - 0.839996315771 , 1 - 0.934417107521 )  ( 1 - 0.84999979977 , 1 - 0.938517371954 )  ( 1 - 0.859999279172 , 1 - 0.942615994967 )  ( 1 - 0.869998758575 , 1 - 0.946714617981 )  ( 1 - 0.879998237977 , 1 - 0.950813240995 )  ( 1 - 0.88999771738 , 1 - 0.954911864008 )  ( 1 - 0.899997196782 , 1 - 0.959010487022 )  ( 1 - 0.909996676184 , 1 - 0.963109110035 )  ( 1 - 0.919996155587 , 1 - 0.967207733049 )  ( 1 - 0.929999639586 , 1 - 0.971307997481 )  ( 1 - 0.939999118989 , 1 - 0.975406620495 )  ( 1 - 0.949998598391 , 1 - 0.979505243509 )  ( 1 - 0.959998077793 , 1 - 0.983603866522 )  ( 1 - 0.969997557196 , 1 - 0.987702489536 )  ( 1 - 0.979997036598 , 1 - 0.991801112549 )  ( 1 - 0.989996516 , 1 - 0.995899735563 )
	(0,0) 
	
};

\addplot[gray!50] fill between[of=perfectEquality and lorenz];


%\legend{Perfect Equality,Perfect Inequality,Lorenz Curve} 
\end{axis}
\end{tikzpicture}


%\vspace{-.05in}
\begin{tikzpicture} 
\begin{axis}[%
hide axis, height =.75in,
xmin=0,xmax=50,ymin=0,ymax=0.4,
legend style={at={(0.5,1)},%0.5)},
	anchor=north,legend columns=-1,column sep=.05cm,draw=none},   
] 
\addlegendimage{black,solid, thick}
\addlegendentry{Perfect Equality}; 
\addlegendimage{black,densely dotted, thick}
\addlegendentry{Perfect Inequality}; 
%\addlegendimage{black,dashed, thick}
%\addlegendentry{Lorenz Curve}; 
\end{axis}
\end{tikzpicture}

\vspace{-.05in}
\begin{tikzpicture} 
\begin{axis}[%
hide axis, height =.75in,
xmin=0,xmax=50,ymin=0,ymax=0.4,
legend style={at={(0.5,1)},%0.5)},
	anchor=north,legend columns=-1,column sep=.05cm,draw=none,fill=none},   
]  
\addlegendimage{black,dashed, thick}
\addlegendentry{Example Lorenz Curve}; 
\end{axis}
\end{tikzpicture}


